Draft Auctions

We introduce draft auctions, which is a sequential auction format where at each iteration players bid for the right to buy items at a fixed price. We show that draft auctions offer an exponential improvement in social welfare at equilibrium over sequential item auctions where predetermined items are auctioned at each time step. Specifically, we show that for any subadditive valuation the social welfare at equilibrium is an $O(\log^2(m))$-approximation to the optimal social welfare, where $m$ is the number of items. We also provide tighter approximation results for several subclasses. Our welfare guarantees hold for Bayes-Nash equilibria and for no-regret learning outcomes, via the smooth-mechanism framework. Of independent interest, our techniques show that in a combinatorial auction setting, efficiency guarantees of a mechanism via smoothness for a very restricted class of cardinality valuations, extend with a small degradation, to subadditive valuations, the largest complement-free class of valuations. Variants of draft auctions have been used in practice and have been experimentally shown to outperform other auctions. Our results provide a theoretical justification.

==> additive-and-unit.tex <==
% !TEX root = draft.tex

Here, we show a larger lower bound on the pure PoA for draft auctions
than we have in the unit-demand case.

\begin{obs}
  The price of anarchy for many-item draft auctions, when there are
  both unit-demand bidders and additive bidders, is at least $4/3$.
\end{obs}
\begin{proof}
  Suppose there are $m$ identical items, one additive bidder with
  value $v$ for each item, and $k$ identical unit-demand bidders each
  with value $p < v$ for any one of the $m$ items. The additive bidder
  must pay at least $p$ for each item if she doesn't allow each $k$
  unit-demand bidders to win items in equilibrium. 

  Thus, if the payoff for the additive bidder is the same whether she
  wins all $m$ items for price $p$ or winning $m-k$ items for free,
  the reciprocal of price of anarchy will be at most $X = \frac{(m-k)v +
    kp}{mv}$. The constraint will be $m(v-p) = v(m-k)$, which then implies
  $\frac{p}{v} = \frac{k}{m}$.

  If we substitute this relation into the objective function $X$, we get

  \begin{eqnarray*}
    X & = & \frac{(m-k)v + kp}{mv}\\
    & = & 1 - \frac{k}{m} + \frac{kp}{mv}\\
    & = & 1 = \frac{p}{v} + \frac{p^2}{v^2}\\
  \end{eqnarray*}

  Minimizing this equation, $\frac{p}{v} = \frac{1}{2}$ yields a price
  of anarchy of $4/3$.
\end{proof}


In the case of single-item auctions with additive and unit-demand
bidders, the price of anarchy is $\Theta(m)$. Here, we present a
$O(\log(m))$ bound on the PoA for the case of many-item draft auctions
with a combination of additive and unit-demand bidders. This is in
contrast with the fact that, for additive bidders, draft auctions are
efficient, and we show a bound of $2$ for the PoA for unit-demand
bidders.

\begin{thm}\label{thm:logapprox}
  The pure PoA for many-item draft auctions is $O(\log(m))$
  when the bidders are either additive or unit-demand.
\end{thm}


\begin{lem}\label{lem:unitdev}
  Any unit-demand bidder has a deviation which can achieve at least
  $\frac{\valopt{i}}{2} - \max\left\{p_{j(i)}, p_{\jopt{i}}\right\}$.
\end{lem}
\begin{proof}
  By the Nash inequality, it is the case that, for any equilibrium
  $s$, and any deviation $s'_i$,

\begin{eqnarray}
  u_i(s_i, s_{-i}) & \geq & u_i(s'_i, s_{-i})
\end{eqnarray}

In particular, either it is the case that $i$ wins when $\jopt{i}$ is
still available or not. If $\jopt{i}$ is still available, we have
$v_{j(i)} \geq \valopt{i}$ which implies

\begin{eqnarray}
u_i(s) &=& v_{ij(i)} - p_{j(i)}\\
& \geq & \valopt{i} - p_{j(i)}\\
& \geq & \frac{\valopt{i}}{2} - p_{j(i)}\\
& \geq & \frac{\valopt{i}}{2} - \max\{p_{j(i)}, p_{\jopt{i}}\}\\
\end{eqnarray}

as desired.

If not $\jopt{i}$ is not available by the time $i$ wins at
equilibrium, she could deviate by bidding $\frac{\valopt{i}}{2}$ at
each round until $\jopt{i}$ is no longer available. If this does not
cause her to win $\jopt{i}$, this implies that
\[p_{\jopt{i}} >\frac{\valopt{i}}{2}\]

and her utility from this deviation is $0$, so if she loses

\begin{eqnarray}
u_i(s'_i, s_{-i}) &=& 0\\
 &\geq & \frac{\valopt{i}}{2} - p_{\jopt{i}}
\end{eqnarray}.

If she does win $\jopt{i}$ by this deviation, then her utility gained
by this deviation is

\begin{eqnarray}
u_i(s'_i, s_{-i})  &=& \valopt{i} -\frac{\valopt{i}}{2}\\
&=&\frac{\valopt{i}}{2}\\
& \geq & \frac{\valopt{i}}{2} - p_{\jopt{i}}
\end{eqnarray}

In either case, her utility from the deviation $s'_i$ is at least

\[u_i(s'_i, s_{-i}) \geq \frac{\valopt{i}}{2} - p_{\jopt{i}}\]

\end{proof}

\begin{lem}\label{lem:adddev}
  Any additive bidder has a deviation which can achieve utility at
  least

  \[\frac{1}{4\log{m}} \svalopt{i} -\sum_{j\in \sjopt{i}}p_j -
  \sum_{j\in \sj{i}}p_j\]
\end{lem}

\begin{proof}
  Consider a bidder $i$. We will show there is a set of items with
  high value for $i$, which he could purchase in addition to (some of)
  the items he purchases at equilibrium.


  Sort the items in $\sjopt{i}$ according to the values $i$ has for
  them, $v_{i1} \geq v_{i2} \geq \ldots \geq v_{im_i}$. Consider the
  partition of items $\mathcal{I}$ where $I_1 = \left\{j : v_{ij} \geq
    \frac{v_{i1}}{2}\right\}$, and more generally, for any $t\in
  \left[2, \log(m)\right]$

 \[I_t = \left\{j \mid \frac{v_{i1}}{2^{t-1}} > v_{ij} \geq
     \frac{v_{i1}}{2^t}\right\}\]


   Let the final set $I_f$ contain all the smallest items, $I_f =
   \left\{j : v_{ij} < \frac{v_{i1}}{m}\right\}$. Notice that the
   largest-valued item in $I_f$ has value at most $\frac{v_{i1}}{m}$
   and there are at most $m-1$ items in $I_f$, thus, $v_{iI_f} <
   v_{i1}$, and so $v_{iI_1} > v_{iI_f}$.

   There are at most $\log(m)$ sets in $\mathcal{P}$, so at least one
   of them has value at least $\frac{\svalopt{i}}{\log(v_{i1})}$
   \emph{from the set $\sjopt{i}$}.  If it is the case that $I_f$ is
   such a set, then so is $I_0$: we will assume our deviation will
   purchase $I_0$ rather than $I_f$ in this case. Let the set of high
   value be denoted $I_{t*}$ and suppose $\mid I_{t*} \mid = k$. Sort
   the items in $I_{t*}$ according to their selling prices at
   equilibrium, $p_1 \geq p_2 \geq \ldots \geq p_{k}$.

   Consider the following deviation for player $i$: emulate $s_i$
   until the first point the winning price is at most $p_{k/2}$. Bid
   $p_{k/2}$ and, upon winning, take $k/2$ items from $I_{t*}$. There
   will still be at least $k/2$ items from $I_{t*}$ remaining, since
   this price was the median price for items from $I_{t*}$. The total
   price for this deviation is at most $1/2 \sum_{j\in I_{t*}} p_j$.

   Recall that $i$ is additive.  Since any two items $j, j'\in I_{t*}$
   have the property that $v_{ij} \geq \frac{v_{ij'}}{2}$, any set of
   size $k/2$ has a sum of values at least $1/4$ of the whole
   set. Thus, the value $i$ will achieve from any set of size $k/2$
   from $I_{t*}$ is at least $\frac{1}{4}v_{i I_{t*}} \geq
   \frac{1}{4\log{m}}$.

   Then, the utility for player $i$ for this deviation will be at
   least

\begin{eqnarray}
  u_i(s'_i, s_{-i}) & \geq  -\sum_{j\in \sj{i}} p_j + \frac{\svalopt{i}}{4\log{m}} - \sum_{j\in \sjopt{i}} \frac{p_j}{2}
\end{eqnarray}
\end{proof}

Now, armed with Lemmas~\ref{lem:unitdev} and~\ref{lem:adddev}, we can
prove Theorem~\ref{thm:logapprox}.

\begin{proof}[Proof of Theoream~\ref{thm:logapprox}]

  Consider the bound we get on each player from
  Lemmas~\ref{lem:unitdev} and~\ref{lem:adddev}. For a unit demand
  bidder $i$, we have

\begin{eqnarray}
u_i(s) & \geq & u_i(s'_i, s_{-i})\\
& \geq & \frac{\valopt{i}}{2} - \max\left\{p_{\jopt{i}}, p_{j(i)}\right\}\\
& \geq & \frac{\valopt{i}}{2} - p_{\jopt{i}} - p_{j(i)}\\
& \geq & \frac{\valopt{i}}{4\log{m}} - p_{\jopt{i}} - p_{j(i)}
\end{eqnarray}

where the second last inequality comes from the fact that prices are
non-negative, and the last inequality holds for sufficiently large $m$.

Thus, the lower bound we have on each player's utility at equilibrium
is the same. Adding this bound over all players, we have

\begin{eqnarray}
  \sum_i u_i(s) & \geq &  u_i(s'_i, s_{-i})\\
  &\geq & - \sum_i \sum_{j\in \sj{i}} p_j - \sum_i \sum_{j\in \sjopt{i}} p_j + \sum_i \frac{\svalopt{i}}{4\log{m}}\\
    & \geq & - 2 REV_{EQ} + \frac{1}{4\log{m}}SW_{OPT}
\end{eqnarray}


The last inequality comes from the fact that the players win different
items at equilbrium, and each of their deviations win at different
prices. Thus, we have

\begin{eqnarray*}
\sum_i u_i(s) = SW_{EQ} - REV_{EQ} \geq - 2 REV_{EQ} + \frac{1}{4\log{m}}SW_{OPT}
\end{eqnarray*}

Rearranging terms, we have that 

\[SW_{EQ} + REV_{EQ} \geq \frac{1}{4\log{m}}SW_{OPT}\]

Individual rationality implies that $REV_{EQ}\geq SW_{EQ}$, and so

\[SW_{EQ} \geq \frac{1}{8\log{m}} SW_{OPT}\]

\end{proof}



==> complements.tex <==
In this section, we give nearly tight upper and lower bounds for the
price of anarchy of draft auctions when bidders have values that
display complementarities.

\begin{thm}
  The price of anarchy(stability) for draft auctions, where bidders
  have valuations with unrestricted complementarities, is $\theta(m)$.
\end{thm}

\begin{proof}
  Consider 2 bidders. One bidder is single-minded, and wants the set
  of all items $[m]$, for which he has value $m$. Then, suppose there
  is a single unit-demand bidder who has value $1+\epsilon$ for any of
  the $m$ items. The optimal allocation will give all of $[m]$ to the
  single-minded bidder, for social welfare of $m$.

  Unfortunately, for the single-minded bidder to take all items at
  equilibrium, he must pay $1+\epsilon$ for each of the items. But,
  since $m(1+\epsilon) > m$, the single-minded bidder will not be
  willing to win all items. Thus, the unit-demand bidder gets utility
  $1+\epsilon$ and the single-minded bidder gets utility $0$.
\end{proof}


\begin{cor}
  The price of anarchy of draft auctions, where bidders' valuations
  have complementarities which are restricted to size at most $k$, is
  $\Omega(k)$.
\end{cor}

\begin{proof}
  Restrict the size of the set of items which the single-minded bidder
  wants to be of size $k$. The proof is then identical.
\end{proof}

\begin{obs}
  Single-minded bidders with desired sets $S$ of size at most $k$
  always have a deviation where they can achieve their optimal bundle
  and pay at most $k p_h$, where $p_h$ is the price of the most
  expensive item in $S$.
\end{obs}
\begin{proof}
  A bidder can always win a set of items $S$ by winning the first
  auction where any of the items in $S$ is sold, and then buying all
  $k$ items. The price for this set will be at most $k p_h$.
\end{proof}

\begin{cor}
  The price of anarchy for draft auctions with a combination of
  single-minded bidders (whose sets are size at most $k$) and
  unit-demand bidders is at most $k$.
\end{cor}

\begin{thm}
  Suppose all bidders have positive weight complementarities of size
  at most $k$.  Then, the pure PoA for them is $O(k^2\log(m))$.
\end{thm}

\begin{proof}

\jmcomment{broken proof
  Consider a player $i$, and the set $i$ gets at $OPT$, denoted
  $\sjopt{i}$. That set corresponds to some set of goods: the value
  $i$ gets from that set corresponds to the sum of weight of a set of
  hyperedges $H_i$ (where goods are hyperedges of size $1$). Sort
  $H_i$ in order of decreasing weight (corresponding to the value $i$
  has for them). Relabel each $h\in H_i$ such that $w_{ih_1} \geq
  ... \geq w_{ih_{\mid H_i \mid}}$. Define the extension of $v_i :
  2^{H} \to \mathbb{R}$ as $v_i(X) = \sum_{h_j \in X} w_{ih_j}$.
  Partition the hyperedges $H_i$ such that $\mathcal{I}$ where $I_1 =
  \left\{h_j : w_{ih_j} \geq \frac{w_{ih_1}}{2}\right\}$, and more
  generally, for any $t\in \left[2, \log(m^k) - 1\right]$

  \[I_t = \left\{h_j \mid \frac{w_{ih_1}}{2^{t-1}} > w_{ih_j} \geq
    \frac{w_{ih_1}}{2^t}\right\}\]


  Let the final set $I_f$ contain all the smallest items, $I_f =
  \left\{j : w_{ih_j} < \frac{w_{ih_1}}{m^k - 1}\right\}$. Notice that
  the largest-valued item in $I_f$ has value at most
  $\frac{w_{ih_1}}{m^k - 1}$ and there are at most $m^k$ items in
  $I_f$, thus, $v_{iI_f} < w_{i1}$, and so $v_{i}(h_1) > v_i(I_f)$.
  There are at most $\log(m^k) = k\log(m)$ sets in $\mathcal{P}$, so
  at least one of them has value at least
  $\frac{\svalopt{i}}{k\log(m)}$. Let $\tau =\argmax_{[t \in 1,
    \ldots, f-1]} v_i(I_t)$, then we have

  \[v_i(I_\tau) \geq \frac{\sjopt{i}}{k\log(m) - 1}\]

  Now, sort the hyperedges in $I_\tau$ by the price of the most-expensive 



\begin{align*}
SW_{EQ} - REV_{EQ} = \sum_i u_i(b)\\
& \geq & \sum_i u_i(b'_i, b_{-i})\\
& \geq & \sum_i \frac{OPT_i}{4\log(m)} - P_i - k p_{i*}\\
& \geq & \frac{SW_{OPT}}{4\log(m)} - (k+1)REV_{EQ}
\end{align*}

Then, rearranging terms and using individual rationality completes the
proof.
}
\end{proof}



==> inefficiency.tex <==
% !TEX root=draft.tex
\subsection{Inefficiency:  Proof of Theorem ~\ref{thm:lowerbounds}}

In this section, we show that draft auctions for unit demand bidders
may be inefficient, even when all players agree on the relative
ordering of the items by their value. We also show that the pure price
of anarchy is between $2$ and $209/177 > 1.22$ for unrestricted
unit-demand bidders. Here, we present an example of the inefficiency
which arises from the competition between agents.

The inefficiency of arbitrary subgame perfect equilibria suggests a
new conjecture: is the price of stability $1$? Our example also shows
the price of stability is strictly larger than $1$, even when all
bidders share the same ranking of the items by value. Indeed, the
example we give below also shows a setting \emph{in which no
  equilibrium is optimal}.

\begin{lem}\label{lem:stability}
  The price of stability for unit-demand bidders in draft auctions is
  strictly larger than $1$, even when all bidders share the same
  ordering of items by value. This implies that the price of anarchy
  is also greater than $1$.
\end{lem}

\begin{figure}
\centering
%\input{inefficiency.pstex_t}
\caption{An example of inefficiency in draft auctions for unit-demand bidders}\label{fig:inefficient}
\end{figure}

%\definecolor {processblue}{cmyk}{0.96,0,0,0}
%\begin{figure}\label{fig:inefficient}
%\begin{center}
%\begin {tikzpicture}[-latex,scale=0.6,every node/.style={scale=0.6},auto ,node distance =2 cm and 4cm ,on grid ,
%semithick , font=\small,
%state/.style ={ circle ,top color =white , bottom color = processblue!20 ,
%draw,processblue , text=blue , minimum width =.5 cm}]
%\node[state] (C)
%{$1$};
%\node[state] (A) {$1$};
%\node[state] (B) [below =of A] {$2$};
%\node[state] (C) [below =of B] {$3$};
%\node[state] (D)  [below =of C] {$4$};
%\node[state] (E) [right = of A] {$a$};
%\node[state] (F) [below =of E] {$b$};
%\node[state] (G) [below =of F] {$c$};
%\node[state] (H)  [below =of G] {$d$};
%\path (A) edge [bend left =0, very near start] node[above] {$1$} (E);
%\path (A) edge [bend left =0, very near start] node[above] {$1 - 2\epsilon$} (F);
%\path (A) edge [bend left =0, very near start] node[below] {$1- 2\epsilon$} (G);
%
%\path (B) edge [bend left =0, very near start] node[above] {$1$} (E);
%\path (B) edge [bend left =0, very near start] node[above] {$1$} (F);
%
%\path (C) edge [bend left =0, very near start] node[above] {$1$} (E);
%\path (C) edge [bend left =0, very near start] node[above] {$1$} (F);
%\path (C) edge [bend left =0, very near start] node[above] {$1- \epsilon$} (G);
%
%\path (D) edge [bend left =0, very near start] node[above] {$1$} (E);
%\path (D) edge [bend left =0, very near start] node[above] {$1$} (F);
%\path (D) edge [bend left =0, very near start] node[above] {$2\epsilon$} (G);
%\path (D) edge [bend left =0, very near start] node[above] {$2\epsilon$} (H);
%
%\end{tikzpicture}
%\end{center}
%\caption{An example of inefficiency in draft auctions for unit-demand bidders}
%\end{figure}
\begin{proof}
The example shown in Figure~\ref{fig:inefficient} has no equilibrium
where the optimal allocation is given. The optimal allocation is
$(a,A), (b,B), (c,C), (d,D)$, with a total weight of
$3+\epsilon$. Since the agents have the same ordering on items, item
$a$ will be selected first. So, for the optimal allocation to be an
equilibrium, $a$ must win the first round.  Then, assuming in the
subgame where $(a,A)$ is removed that the optimal allocation is
reached and solving for prices, the price vector for such an
allocation is $(1-2\epsilon, 1-2\epsilon, 0,0)$, where player $b$
price-sets in the first round and player $d$ price-sets in the second round\footnote{ We can ensure $b$ is the price-setter for player $a$ by
  slightly increasing the weight on the edges $(b,A)$. That way, $b$
  will have a slightly higher incentive to beat $a$ than $d$ has.}.
Thus, player $a$ gets utility $2\epsilon$ from winning the first
round.

Now, consider what happens if $a$ loses the first round to player $b$. If we
assume in any subgame, the optimal allocation is the one which is
made, the allocation in the subgame will be $(a,C), (c,B),
(d,D)$. Then, $c$ will pay $1-2\epsilon$, and $a$ will pay nothing,
for utility $1-2\epsilon$. So, if $a$ chooses to lose to player $b$,
her utility is $1-4\epsilon$ higher than if she won the first round.

\end{proof}

\begin{lem}\label{lem:lower}
  The pure price of anarchy of draft auctions for unit-demand bidders
  is at least 1.22.
\end{lem}

\begin{proof}

Consider the matrix

\[ \left( \begin{array}{c|ccc}
A & 32 & 31 & 83 \\
B & 9 &  84&  97\\
C & 2 & 42 & 93 \end{array} \right)\] 

and the strategy profile where $B$ wins first, supported by price
$p_1 = 51$ by agent $A$, then $C$ wins at price $p_2 = 0$, then $A$
wins at price $p_3 = 0$. The allocation will be $(1, 3, 2)$, with
social welfare $97 + 32 + 42 = 171$, while the optimal allocation
$(1,2,3)$ gives social welfare of $32 + 84 + 93 = 209$. Thus, the PoA is
at least $209/171 > 1.22$.


Showing this is a SPE is not difficult: it is necessary, however, for
$A$ to be the price supporter in round 1, rather than $C$ (both have
equal externality for $B$ winning round 1). if $C$ price-sets, $B$
would rather lose round $1$ and the outcome will be efficient.
\end{proof}

%\jmdelete{Consider the following proposed strategy. In each round $t$, compute
%the maximum Walrasian price on the remaining items and
%bidders. Consider the highest-priced item $j_t$, its winner $i_t$, and
%its price-setter $i'_t$, with price $p_t$. The joint strategy, at time
%$t$, for $i_t$ to bid $p_t+$, $i'_t$ to bid $p_t$ (all other bidders
%bid $0$), and for $i_t$ to select item $j_t$ when she wins, is
%\emph{not an equilibrium in undominated strategies}. Moreover, it is
%not an equilibrium at all.
%
%On the other hand, for this example utility matrix, there is still an
%equilibrium without overbidding which implements the efficient
%outcome.
%
%
%The idea is that the price-supporter in the original Walrasian
%equilibrium may be a price-setter at $p_t$ \emph{because her item has
%  some price $p_{t'} > 0$}, but in the draft auction, she gets this
%item for less than $p_{t'}$; in our example, she can win her item for
%$0$, meaning that price-setting at that same price would be
%overbidding for her.
%
%\ndcomment{What is the following a proof of? State it as a lemma. } 
%\begin{proof}
%Consider the following matrix of values:
%
%
%\[ \left( \begin{array}{c|cccc}
%a & 0 & 0 & 53 & 62 \\
%b & 0 & 63 & 59 & 0\\
%c & 55 & 66 & 0 & 0\\
%d & 0 & 0 & 66 & 72  \end{array} \right)\] 
%
%The optimal allocation is $(3,1,0,2)$; player $a$ gets item $3$ and so
%on.  The Walrasian prices for this allocation are $(13, 11, 0, 7)$
%(ordered by winner, not item; player $a$ pays $13$, player $b$ pays
%$11$, player $c$ pays $0$, and player $d$ pays $7$). Player $d$ is the
%supporter of the price $13$ for player $a$, since $d$ gets utility
%$59$ from her allocation/price pair, but could get $72 - p_a$ if she
%outbid $a$, so $p_a \geq 13$.
%
%However, if we consider the draft auction, once players $a$ and $b$
%win their items, players $c$ and $d$ don't price-set for each other,
%since they each have their own favorite remaining item (whereas in the
%Walrasian equilibrium, player $b$ price-set for player $d$).  Then,
%player $d$ could win $2$ for price $0$, getting utility $66$ from
%that. So, it would be overbidding for her to bid $13$ in the first round.
%
%Moreover, it is not an equilibrium for $a$ to win at price $13$, if
%everyone is using the aformentioned strategy in every subgame. If $a$
%loses to $d$ in round $0$, $d$ takes item $3$. Then, $b$ pays $11$ for
%item $1$, supported by $c$. Then, $a$ gets $2$ and $c$ gets $0$, both
%for free.  So, the utility $a$ gets from this deviation is $53$, which
%is larger than $62 - 13 = 49$.
%
%The first price also must be at least $11$, if there is an equilibrium
%where the max-weight matching is the allocation, since player $c$ gets
%an item he values $11$ less than his max-valued item at equilibrium.
%Either player $a$ or $b$ must win the first round in any equilibrium
%which implements the efficient outcome, since they are the two bidders
%who get their favorite items.
%dr
%All that remains is to show an equilibrium which implements the
%efficient outcome, without overbidding. Suppose we consider $c$'s
%strategy to bid $11$ in rounds $1$ and $2$, but lose to $a$ and then
%$b$, respectively. In this case $a$ gets her favorite item, for
%utility $u_a = 62 -11 = 51$, $b$ gets his favorite item for utility
%$u_b = 63 -11 = 52$, and then $c$ and $d$ pay nothing but get utility
%$u_c = 55$, $u_d = 66$.
%
%If $a$ were to lose to $c$, the subgame that would be induced is
%
%\[ \left( \begin{array}{c|ccc}
%a & 0  & 53 & 62 \\
%b & 0  & 59 & 0\\
%d & 0 & 66 & 72  \end{array} \right)\] 
%
%And, in this subgame, either $a$ will get an item she values $0$, or
%she must pay at least $59$, implying that she'll get no more utility
%than $3$. So she'd rather win than let $c$ win in the first round.
%
%If $b$ were to lose to $c$ in the next round, a similar thing would
%happen: the subgame $b$ would find himself in would be
%
%\[ \left( \begin{array}{c|cc}
%b & 0  & 59 \\
%d & 0 & 66  \end{array} \right)\] 
%
%And $b$ can no utility from such a subgame.
%
%Thus, $a$ and $b$ winning the first rounds for price $11$, supported
%by player $c$, and $c$, $d$ winning the final rounds for free, is an
%equilibrium (and implements the efficient allocation).
%
%
%\end{proof}
%}
%
The proof of Theorem~\ref{thm:lowerbounds} follows from Lemma~\ref{lem:stability} and Lemma~\ref{lem:lower}.


==> multi-unit.tex <==
% !TEX root = draft.tex
Consider now the setting where we have $m$ identical copies of an
item. In this setting, each bidder $i$ has a valuation function $v_i:
\mathbb{N}\to \mathbb{R}$ which is concave in the number of items
they receive. 

\begin{lem}
  The pure price of anarchy for selling $k$ identical items is
  $4$ for any pure subgame perfect equilibrium $s$.
\end{lem}
\begin{proof}

  Consider the sequence of selling prices $p_1, \ldots, p_k$, with
  multiplicity given to those prices where multiple items were
  sold. Sort them in descending order, such that $p'_1 \leq p'_2 \leq
  \ldots \leq p'_k$. Let $\optall$ denote the number of copies bidder
  $i$ is allocated in $OPT$.

  The, consider the following strategy for player $i$ to deviate. If
  $i$ wins at least $\optmid$ copies according to $s$, follow $s$. If
  not, bid according to $s$ until the first time $t$ at which the
  price $p_t \leq \poptmid$. At that time, bid $\poptmid$
  and buy $\optmid$ items at that price. First, notice there will still
  be at least $\optmid$ copies left to purchase, since there are at
  least $\optmid$ copies sold at prices lower than $\poptmid$
  (and, by assumption, this is the first point at which the price was
  at most that value). Call this strategy $s'_i$. By the
Nash inequality, we know that 

\begin{eqnarray}
  u_i(s) &\geq& u_i(s'_i, s_{-i})\label{nash}
\end{eqnarray}


  Let $win_i$ be the set of auctions $i$ wins according to $s$ and
  $n_j$ be the number of items bought at time $j$. Now, consider the
  utility player $i$ gets from such a deviation:

\begin{eqnarray*}
  u_i(s'_i, s_{-i}) &\geq& v_i(\optmid) - \sum_{j\in win_i}p_j n_j - \poptmid\optmid \\
&\geq & 1/2 v_i(\optall) - \sum_{j\in win_i}p_j n_j - \poptmid\optmid 
\end{eqnarray*}

where the inequality comes from the fact that not all bidders will
need to buy copies beyond those that they purchased according to $s$,
and the second inequality comes from the concavity of $v_i$. 

Then, if we sum over all $n$ bidders, notice that $\sum_i \optmid =
k/2$, and that, for all $i$, $\poptmid \leq \frac{2 REV_{EQ}}{k}$,
since $\poptmid \leq p_{k/2} \leq \frac{2 REV_{EQ}}{k}$. Thus,
summing over all bidders we have

\begin{eqnarray}
 \sum_i u_i(s'_i, s_{-i}) &\geq& 1/2 SW_{OPT} -  REV_{EQ} - REV_{EQ} \label{fin}
\end{eqnarray}

Combining ~\ref{nash} (summed up over all $i$) and ~\ref{fin}, we have
that

\begin{eqnarray}
SW_{EQ} - REV_{EQ} \geq 1/2 SW_{OPT} - 2 REV_{EQ}\\
SW_{EQ} \geq 1/2 SW_{OPT} - REV_{EQ}\\
4SW_{EQ} \geq  SW_{OPT}
\end{eqnarray}

\end{proof}
























==> old-intro.tex <==

Suppose there are $n$ bidders and $m$ items we wish to sell. We are
interested in developing simple mechanisms to do so, with good
properties with respect to social welfare and revenue.  If the items
are held by different owners, or if we wish to surpass the unbounded
price of anarchy for running sequential first-price auctions in the
setting of bidders whose valuations are more general than unit-demand,
it may make sense to consider new, simple mechanisms which require
little coordination between the items' sellers.

Here, we analyze the following mechanism, which we call \emph{
  sequential draft auctions}. The sequential draft auction will, in
each round, run a first-price auction; the winner, who bid $b$, can
select any set of items $S$ and will pay $b \mid S \mid$ for those
items. The remaining items will be sold in the following rounds. We
will consider subgame perfect equilibria of these games which survive
iterative removal of dominated strategies. We will also describe
\emph{single draft auctions}, where the winning bidder in each round
is restricted to buying only one item for price $b$.

==> old-preliminaries.tex <==
% !TEX root=draft.tex

In this work, we introduce a new auction mechanism, which we call
\emph{sequential draft auctions}.  Let $m$ be the number of items for
sale and $n$ the number of bidders. Each bidder has a combinatorial
valuation function $v_i: 2^{[m]} \to \mathbb{R^+}$ which we assume to
be monotone \vsdelete{(agents are not made less happy by winning additional
items)}. We assume that players have quasilinear utility, i.e. player $i$'s
utility for a set $S$ and a total payment of $p_i$ has the form $u_i(S,p) = v_i(S) - p_i$.

\begin{mdef}[Draft Auction]
  In the \emph{single-item sequential draft auction}, there are $m$
  rounds. Initially, the set of available items $I^0 = [m]$. In each
  round, the mechanism runs a first-price auction. The strategy space
  in round $t$ for player $i$ is $[0, \infty) \times I^t$, a bid and an item.
  Let the bid tuple in round $t$ be $(b^t_1, \ldots, b^t_n)$ and the
  item tuple be $(x^t_1, \ldots, x^t_n)$.  The winner $i =
  \argmax_{i'} b^t_i$ pays $b^t_i$ and wins $x^t_i$. Then, $I^{t+1} =
  I^t\setminus \{x^t_i\}$.

  For the most general \emph{sequential draft auction}, there will
  again be a first-price auction amongst all $n$ bidders in each round
  and $I^0 = [m]$. The strategy space in round $t$ is $[0, \infty]
  \times 2^{I^t}$, a bid and a collection of items. Let $(X^t_1,
  \ldots, X^t_n)$ be the tuple of demanded items. If $i$ is the
  winner, $i$ pays $b^t_i \times \mid X^t_i \mid$ and wins
  $X^t_i$. Then, $I^{t+1} = I^t \setminus X^t_i$.
\end{mdef}

Let us assume there is some fixed tie-breaking order, and that players
can bid $b+$, a bid which beats any bid $b$ but whose payment is
$b$. These bids are necessary for best response moves to exist in
first-price auctions. 

We analyze the set of \emph{subgame perfect equilibria} of draft
auctions, the sequential analogue of Nash equilibrium.

\begin{mdef}
  Consider a tuple of strategies $s = (s_1, \ldots, s_n)$ where $s_i$
  is a funtion from nodes in the game tree to actions for player
  $i$. The tuple $s$ is \emph{subgame perfect equilibrium} of a game
  if, for any node $t$ in the game tree, fixing the path to $t$, the
  tuple $(s_1(t), \ldots, s_n(t))$ is a Nash equilibrium in the
  induced game.
\end{mdef}

Let $s$ be any tuple of bidding strategies. Let $S_i$ be the set of
items player $i$ wins if everyone plays according to $s$ (in the case
of mixed strategies, $S_i$ will be a random variable). The
\emph{social welfare} of the allocation $S$ is $SW(s) = \sum_i
v_i(S_i)$. We also use the notation $REV$ to denote the total revenue
of a strategy. We will analyze sequential draft auctions in terms of
their social welfare at subgame perfect equilibrium, and use the
optimal allocation as a benchmark. In particular, we will consider the
\emph{Price of Anarchy} for a set of equilibria $T$:

\[ PoA(T) = \max_{s\in T}\frac{SW(OPT)}{SW(s)}\]

where $T$ may be the restriction to pure subgame perfect equilibria,
or the whole set of subgame perfect equilibria, or the set of
Bayes-Nash equilibria, or the set of correlated equilibria. We will
also consider the \emph{Price of Stability} for a set of equilibria $T$:

\[ PoS(T) = \min_{s\in T}\frac{SW(OPT)}{SW(s)}\]

since the best equilibrium may have substantially higher social
welfare than the worst equilibrium. We note that for single-item draft
auctions, pure subgame perfect equilibria are guaranteed to exist, by
a simple extension of the argument made in previous work studying
sequential item auctions~\cite{pureseq}. There is not a simple
extension to the argument which works for general draft auctions.


The analysis of Bayes-Nash and mixed subgame perfect equilibria for
draft auctions follow the smoothness framework introduced in previous
work~\cite{smoothmech}, which allows a bound on the pure price of
anarchy to extend to these more general settings if the proof is of a
certain form.

TODO(jamiemmt): outline of organization. Do after we've reorganized things.
\subsection{Restrictions on valuation functions}

Our results in the paper show bounds on the price of anarchy of draft
auctions with various restrictions on the valuation functions of
players. The multi-unit setting is one where there
are $k$ identical copies of an item. Each $v_i$ is assumed to be
concave in the number of items allocated to player $i$.

If $v_i (S_i) = \max_{t\in S_i} v_i(t)$, for all $S_i$, we say $v_i$
is unit-demand. If $v_i(S_i) = \sum_{t\in S_i} v_i(t)$ for all $S_i$,
$v_i$ is an additive valuation function. If $v_i(S \cup T) \leq v_i(S)
+ v_i(T)$ for all $S, T$, then $v_i$ is said to be subadditive. If
$v_i$ is representable as a maximum of linear functions over sets of
items, e.g. $v_i(S) = \max\{\sum_{j\in S}v_{1j}, \ldots, \sum_{j\in
  S}v_{kj}\}$, then $v_i$ is said to belong to the set of $XOS$
valuation functions. All of these restricted classes of valuations
belong to the set of valuations with no complementarities.  Here, we
present the heirarchy of such restrictions on valuation functions,
along with other well-known restrictions valuation functions:

TODO(jamiemmt): make this image and cite Nisan paper


We also present results for the class of valuations with
$k$-restricted complementarities (for a formal definition, see
~\cite{complements}), where the hypergraph describing the
complementarities has edges of size at most $k$.


==> old-related.tex <==
% !TEX root=draft.tex
% related.tex

There has been a long line of research on quantifying inefficiency of
equilibria starting from \cite{Koutsoupias1999} who introduced the
notion of the price of anarchy. Several recent papers have studied the
efficiency of simple mechanisms.  A series of papers, Christodoulou,
Kovacs and Schapira \cite{Christodoulou2008}, Bhawalkar and
Roughgarden \cite{Bhawalkar} Hassidim, Kaplan, Mansour, Nisan
\cite{Hassidim2011}, and Feldman et al. \cite{Feldman2013}, studied
the inefficiency of Bayes-Nash equilibria of non-truthful
combinatorial auctions that are based on running simultaneous separate
single-item auctions.  Lucier and Borodin studied Bayes-Nash
Equilibria of non-truthful auctions based on greedy allocation
algorithms \cite{Lucier2009}. Paes Leme and Tardos
\cite{PaesLeme2010}, Lucier and Paes Leme \cite{Lucier2011} and
Caragiannis et al. \cite{Caragiannis2011} studied the ineffficiency of
Bayes-Nash equilibria of the generalized second price
auction. Roughgarden \cite{Roughgarden2009} showed that many price of
anarchy bounds carry over to imply bounds also for learning
outcomes. Roughgarden \cite{Roughgarden2012} and Syrgkanis
\cite{Syrgkanis2012} showed that such bounds also extend to bound the
inefficiency of games of incomplete information. Recently, in
\cite{Syrgkanis2013} gives a more specialized framework for the case
of non-truthful mechanisms in settings with quasi-linear preferences,
showing how to capture several of the previous results. In this work
we show that our upper bounds for correlated and Bayes-Nash equilibria
of the simultaneous auction fall into the framework of
\cite{Syrgkanis2013}. 

In the context of a sequence of auctions, another line of
work~\cite{judaoptions} has aimed to design mechanisms for which
truth-telling is a dominant strategy. In particular, this work focuses
on the the combination of the exposure problem (bidders' inability to
purchase complements together), the multiple copies problem (bidders'
inability to ensure they purchased the cheapest copy of a given item),
and temporal issues (not all items are available simultaneously), all
of which lead to non-composable dominant strategies. They use a
price-option mechanism: each bidder submits his valuation, and for
each bidder, a proxy collects options to buy items at various prices,
and then exercises some subset of these options. This proxy causes
truth-telling to be a dominant strategy for bidders.


Our work is most closely related with the recent work on quantifying
the inefficiency in sequential first and second price auctions for
heterogeneous items
\cite{PaesLeme2012,Syrgkanis2012a,Syrgkanis2013}. For sequential
first-price auctions \cite{PaesLeme2012} showed that when bidders are
unit-demand, every subgame perfect equilibrium achieves at least 1/2
of the optimal welfare, while for submodular bidders the inefficiency
can grow with the number of items, even with a constant number of
bidders. The positive results were later extended to the
incomplete-information setting in \cite{Syrgkanis2012a} and to
no-regret outcomes and budget-constrained bidders in
\cite{Syrgkanis2013}. On the negative side, Feldman et
al. \cite{Feldman2013b} showed that even when some bidders are
unit-demand and some are additive then the inefficiency can grow
linearly with the minimum of the number of items and bidders. Our work
shows that such inefficiencies can be largely alleviated by performing
sequential auctions for the option to by some item, rather than for a
specific item. Thereby, our work portrays that it was not the
sequentiality that caused the inefficiency but rather the specific
ordering of the items being auctioned.

A lot of the work in the economic literature has analyzed sequential
auctions for homogeneous items. Weber \cite{Weber2000} and Milgrom and
Weber \cite{Milgrom1982a} analyze first and second price sequential
auctions with unit-demand bidders in the Bayesian model of incomplete
information and show that in the unique symmetric Bayesian equilibrium
the prices have an upward drift. Their prediction was later refuted by
empirical evidence (see e.g. \cite{Ashenfelter1989}) that show a
declining price phenomenon. Several attempts to describe this
``declining price anomaly'' have since appeared such as McAfee and
Vincent \cite{McAfee1993} that attribute it to risk averse
bidders. Although we study full information games with pure strategy
outcomes, we still observe declining price phenomena in our sequential
auction models without relying to risk-aversion.  Boutilier el al
\cite{Boutilier99} studies first price auction in a setting with
uncertainty, and gives a dynamic programming algorithm for finding
optimal auction strategies assuming the distribution of other bids is
stationary in each stage, and shows experimentally that good quality
solutions do emerge when all players use this algorithm repeatedly.


The multi-unit demands case has been studied under the complete
information model as well. Several papers
(e.g. \cite{Gale2001,Rodriguez2009}) study the case of two bidders. In
the case of two bidders they show that there is a unique subgame
perfect equilibrium that survives the iterated elimination of weakly
dominated strategies, which is not the case for more than two bidders.
Bae et al. \cite{Bae2009,Bae2008} study the case of sequential second
price auctions of identical items to two bidders with concave
valuations on homogeneous items. They show that the unique outcome
that survives the iterated elimination of weakly dominated strategies
is inefficient, but achieves a social welfare at least $1-e^{-1}$ of
the optimal.


Several lines of research in the economics community have studied
draft auctions, under the names of \emph{pooled auctions} or auctions
for the \emph{right to choose}, or RTC auctions.  Empirical
work~\cite{ashenfelter} studied condominium sales, which often proceed
using a draft auction, where the winner selects their favorite condo
which hasn't been selected so far. 37\% of the auction sales fell
through, and the remaining condos were then sold in face-to-face
bargaining. The revenue was substantially higher in the draft auction
(13\% higher). The largest price discount was for those items sold
earliest in the draft auction.  

Later empirical work ~\cite{alevy} studies these "right to choose"
auctions in the context of water rights sales in Chile, and again
finds significantly higher revenue than in the analagous sequential
auction.  When bidders are single-minded, there is more experimental
evidence ~\cite{eliaz} that the revenue of the RTC is larger than the
item-by-item auctions, though theoretically this should not be the
case.

Several other papers ~\cite{goeree, burguet} use synthetic experiments
supporting the case that increase in revenue is due to risk-aversion
of bidders. Other empirical work~\cite{salmon}, however, suggests the
increase in revenue occurs even when risk aversion does not. In the
setting of 2 bidders, Harstad~\cite{harstad} considers the revenue
guarantees for different constraints on the bidding strategies and
valuations of bidders. Theoretically, previous work ~\cite{gale} has
shown that, for 2 unit-demand bidders, all Bayes-Nash equilibria yield
socially optimal allocations.



==> single-value.tex <==
% !TEX root = draft.tex

Consider a restriction of unit-demand bidders, where each bidder $i$
is only interested in some subset of items, and values any one of
these items at value $v_i$ (and has no additional utility for multiple
items).  The following is a direct corollary of Theorem 4.1 of work by
Paes Lemme et. al ~\cite{pureseq}.

\begin{cor}
  In a sequential first-price auction auction for single-unit demand
  bidders, there exists a subgame perfect equilibrium in undominated
  strategies that emulates the VGC outcome.
\end{cor}

\begin{proof}
TODO
\end{proof}

\begin{cor}
   ??TODO??  There was something to say about the incomplete information case?
\end{cor}

==> smoothness_-_old.tex <==
% !TEX root=draft.tex
We will show that draft auctions are smooth mechanisms according to
\cite{Syrgkanis2013} and therefore they achieve good social welfare at
every Correlated Equilibrium of the complete information setting and
every mixed Bayes-Nash equilibrium of the incomplete information
setting.

To prove the smoothness property we need to show that from any current bid profile, every player
has a deviating strategy that depends only on what he was doing previously, such that either he gets utility
that is a constant fraction of his value in the optimal allocation, or his items in the optimal allocation
are currently sold at a high price.

Mainly for expository purposes we begin by analyzing the case of unit-demand bidders. In this setting, 
each player is allocated only one item in the optimal allocation. When moving to multi-unit valuations we also need to cope with the fact that a player needs to acquire many items with his deviation and we explain how to cope with this added difficulty in the next section. For unit-demand bidders, we simply need to show that  a player can always get 
a constant fraction of his value for that item, at its current price. A main technical difficulty in the analysis is that the moment
a player deviates he changes the equilibrium history and thereby he is facing out-of-equilibrium prices, which might be arbitrarily higher. Thus we need to carefully construct a deviation, such that as long as a player is not winning he is not affecting the equilibrium path. 

Additionally, an extra technical difficulty is that unlike sequential item auctions, a player is not aware, in advance, at which step his optimal item is going to be allocated, since this is endogenously chosen by one of his opponents. Thus deviations of the sort: "behave exactly as previously until the optimal item arrives and then deviate to acquire it", are not feasible in the case of draft auctions. In essence, the player must always be on alert and attempting to get his optimal item, without however changing the observed history when he loses. We show that the following high level deviation achieves the effect that we wanted: 
\emph{At each time step, as long as your optimal item is still available, bid the maximum of your equilibrium bid and half your value for your optimal item. If you ever win buy your optimal item.}

\begin{thm}The draft auction for unit-demand bidders is a
  $(\frac{1}{2},2)$-smooth mechanism.
\end{thm}
\begin{proof}
  Consider a valuation profile $v$. We will show that for any $b_i$,
  there exists a $b_i'$, such that for any $b_{-i}$:
\begin{equation}
  u_i(b_i',b_{-i})\geq \frac{1}{2}v_{ij_i^*}-p_{j_i^*}(b)-P_i(b)
\end{equation}
Consider the following $b_i'$: at every auction the player bids the
maximum of his previous bid $b_{ij}$ (conditional on the history) and
$\frac{v_{ij_i^*}}{2}$, until his optimal item gets sold. If he ever
wins some auction he picks his optimal item.

Suppose that player $i$'s optimal item was sold at some auction $t$
under strategy profile $b$. Suppose that under $b$ player $i$ was
winning some auction $t'\leq t$. Then under $b_i'$ he is still
definitely winning that auction since he is bidding at least as
high. Thus in that case he is getting utility
$$u_i(b_i',b_{-i})\geq v_{ij_i^*}-\max\left\{\frac{v_{ij_i^*}}{2},b_{it'}\right\}\geq \frac{v_{ij_i^*}}{2}-P_i(b).$$

Now suppose that under $b$ he is not winning any auction at an item
$t'\leq t$. Then if player $i$ doesn't still win any item at an
auction $t'\leq t$ then when $t$ arrives his deviation is transparent
since it didn't affect the outcomes. Thus if $p_{j_i^*}(b)<
\frac{v_{ij_i^*}}{2}$ then the player must be definitely winning
auction $t$ and getting utility $u_i(b_i',b_{-i})\geq
v_{ij_i^*}-\max\left\{\frac{v_{ij_i^*}}{2},b_{it}\right\}$. He could
have also won some auction $t'\leq t$, but then also in that case:
$u_i(b_i',b_{-i})\geq
v_{ij_i^*}-\max\left\{\frac{v_{ij_i^*}}{2},b_{it'}\right\}$. In any
case, if $p_{j_i^*}(b)<\frac{v_{ij_i^*}}{2}$ then for some $t'\leq t$:
$$u_i(b_i',b_{-i})\geq v_{ij_i^*}-\max\left\{\frac{v_{ij_i^*}}{2},b_{it'}\right\}\geq  \frac{v_{ij_i^*}}{2}-b_{it'}\geq \frac{v_{ij_i^*}}{2}-P_i(b)$$
So either $p_j(b)\geq \frac{v_{ij_i^*}}{2}$ or $u_i(b_i',b_{-i})
+P_i(b)\geq \frac{v_{ij_i^*}}{2}$.  In any case:
\begin{equation}
  u_i(b_i',b_{-i}) \geq \frac{v_{ij_i^*}}{2}-p_{j_i^*}(b)-P_i(b)
\end{equation}
Therefore we see that in any case his utility from this deviation is
lower bounded by the desired bound.

The smoothness property follows by using the mapping described
previously, summing over all players and using the fact that $\sum_i
p_{j_i^*}(b)=\sum_{j\in [m]}p_j(b)=\sum_i P_i(b)$.
\end{proof}

Thus the latter implies that the draft auction has Bayes-Nash and
correlated price of anarchy of at most $4$. This bound is comparable
but not identical to our bound on the pure price of anarchy, which we
show to be upper-bounded by $2$ in the appendix. 

\subsection{Identical Items}

As a next step to general no-complement valuations, we analyze the case where items are identical and players
have valuations that are concave functions of the units they acquire. To analyze such valuations we provide a key
lemma that will be quintessential in subsequent sections too. 

Specifically, we construct a good deviating strategy for a more general class of valuations, where players are only interested in
a subset of the items $S\subseteq [m]$ and treat all items in their interest set homogeneously, i.e. their value is a concave function of the units they acquired from their interest set. We will denote such valuations are \emph{constraint-homogeneous valuations}.

Unlike the unit-demand case, each player will be allocated several units in the optimal allocation. Thus a good deviating strategy should achieve a constant fraction of a player's valuations for his optimal number of units and at a price that is not much larger than what is being paid for those units at equilibrium. Constructing such a deviating strategy is inherently more difficult than in the unit demand case. A player should always be trying to acquire his optimal number units at a good price, whilst at the same time not changing the observed history of play. 

The first idea is that the "right" price that a player should bid to acquire his optimal units is half of the per unit value
assuming he gets the half of the number of units as in his optimal allocation. With such a deviation his goal is to eventually
acquire half of his optimal number of units. To avoid altering the history of play, the player should bid the maximum of his equilibrium bid and this "right" price. However, unlike unit-demand valuations it is not the case that getting all his 
targeted units is the right approach. The reason is that he might have won the auction because his equilibrium bid was really
high. Additionally, it might have been that under the equilibrium he was only getting a single unit at that iteration. Thus by
getting more units at that high price he is overpaying. Instead, the right deviation, gets the same number of units
as under equilibrium, when a player wins because of his equilibrium bid and gets the number of items need to complete the
target number units, whenever a player wins with the "right" price. 

The proof of the Lemma is rather involved and requires arguing that either a player was getting many items at equilibrium or otherwise we can charge the price paid by the user
under the deviation to the prices paid by players who acquired his units under the equilibrium.

\begin{lem}[Core Deviation Lemma]\label{lem:multi-unit}
  Consider a subset of items $S$, that are identical from the
  perspective of a player $i$: i.e. for all $T\subseteq S:
  v_i(T)=v_i(|T|)$ and suppose that player $i$ has a monotone
  valuation over the whole set of items $[m]$. Then in a draft auction
  there exists a deviation mapping $b_i':B_i\rightarrow B_i$ such
  that, for any strategy profile $b$:
$$u_i(b_i'(b_i),b_{-i};v_i)\geq   \frac{1}{2}v_i\left(\frac{|S|}{2}\right)-\sum_{j\in S}p_j-P_i(b)$$
\end{lem}
\begin{proof}
  Consider a bid profile $b$. Let $S$ be a homogeneous set of items
  for player $i$ as described in the theorem. We will refer to the
  items in $S$ as units as opposed to items, which will be any item
  not in $S$. Let $p_j$ be the price that unit $j$ was sold under
  strategy profile $b$. Also re-order the index of the units of $S$
  such that $p_1\leq p_2\leq \ldots \leq p_{|S|}$. This is not
  necessarily the order at which they were sold. Let $t(j)$ be the
  auction at which item $j\in S$ was sold and we denote with $P_t$ the
  price of auction $t$ under bid profile $b$.

  We also make the extra observation that the number of units that a
  player acquires at auction $t$, subject to winning, do not depend on
  the price of the auction since it is completely defined by the bid
  of the player. Additionally, a player doesn't learn anything else
  after the bidding phase.  We will denote with $k_{it}$ the number of
  units of $S$ that player $i$ was obtaining at auction $t$ under bid
  profile $b$ subject to winning.

  Consider the following deviation of player $b_i'$: let
  $b_i^*=\frac{1}{|S|}\cdot v_i\left(\frac{|S|}{2}\right)$ be half the
  average per unit value for $|S|/2$ units of $S$. At every auction
  $t$, he submits $b_{it}'=\max\left\{b_i^*, b_{it}\right\}$. If he
  wins with bid $b_i^*$ then he buys $|S|/2$ minus the number of units
  of $S$ he has already acquired and drops out.  If he wins with a bid
  of $b_{it}$ he buys $k_{it}$ units of $S$ together with any other
  item that he was buying under strategy profile $b_i$ at auction $t$
  and continues to bid until he acquires $|S|/2$ units of $S$ or the number
of units of $S$ remaining are not sufficient for him to complete $|S|/2$ units.

  The crucial observation is that as long as a player hasn't already
  acquired $|S|/2$ units then he is not affecting the game path
  created by strategy profile $b$ in any way, since from the
  perspective of the other bidders either he behaved exactly as under
  $b_i$, by winning at his price under $b_i$ and getting the items he
  would have got under $b$ or he won at a higher price, but then he
  acquired all the units needed to reach $|S|/2$ at the auction where
  he bid higher in the deviation. Thus the prices that he faces in all
  the auctions prior to having won $|S|/2$ units are the same as the
  prices under strategy profile $b$.

  First it is easy to observe that if player $i$ was obtaining at
  least $|S|/2$ units under $b_i$ then he is definitely winning
  $|S|/2$ units under $b_i'$. Moreover he is paying at most
  $\frac{|S|}{2} b_i^* +
  P_i(b)=\frac{1}{2}v_i\left(\frac{|S|}{2}\right)+P_i(b)$. Thus under
  this condition we get that the utility from the deviation is at
  least:
$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{|S|}{2}\right)-P_i(b)$$ 

Thus we can assume that under $b_i$ player $i$ is winning less than
$|S|/2$ units. Let $t^*$ be the first auction that was won at price
$P_{t^*}\leq p_{|S|/2}$ under $b$ and not was not won by bidder
$i$. We know that such an auction must exist since there are $|S|/2$
units that are sold at a price at most $p_{|S|/2}$ and by the
assumption on the limit of units won by player $i$ under $b_i$, some
unit of them was not won by player $i$. Thus one candidate auction for
$t^*$ is the auction that this unit was sold at.

If player $i$ has already won $|S|/2$ units prior to $t^*$ then the
same lower bound of $\frac{1}{2}v_i\left(\frac{|S|}{2}\right)-P_i(b)$
on the deviating utility holds. Thus we can assume that the player has
not won $|S|/2$ units prior to $t^*$ and hence he is still
bidding. Let $k_{i,<t^*}$ be the number of units acquired by player
$i$ prior to $t^*$. Observe that by the definition of $t^*$ there are
at least $|S|/2-k_{i,<t^*}$ units available for sale at that
auction. This follows from the fact that for any auction $t<t^*$ for
which $P_t\leq p_{|S|/2}$, we know that player $i$ was winning under
$b_i$. Thus every unit that was sold prior to $t^*$ at a price of less
than or equal to $p_{|S|/2}$ was sold to player $i$. There are $|S|/2$
units sold at a price $\leq p_{|S|/2}$ and the number of such units
sold prior to $t^*$ is at most the number of total units allocated to
bidder $i$ prior to $t^*$. Thus the number of available units
available at $t^*$ is at least: $|S|/2-k_{i,<t^*}$.

If $P_{t^*}<b_i^*$, then player $i$ is winning auction $t^*$. Since he
was not winning $t^*$ under $b_i$, it must be that he is winning $t^*$
with a bid of $b_i^*$. Thus at that auction he will buy every unit
needed to reach $|S|/2$ units. By the analysis in the previous
paragraph, we know that there are still enough units available for
sale to reach $|S|/2$. Thus in this case he will win $|S|/2$ items and
pay at most $\frac{|S|}{2} b_i^* + P_i(b)$. Therefore, we get that his
utility from the deviation is also at least:
$\frac{1}{2}v_i\left(\frac{|S|}{2}\right)-P_i(b)$.

Thus the above analysis states that either $P_{t^*}\geq b_i^*$ or
$u_i(b_i',b_{-i})\geq
\frac{1}{2}v_i\left(\frac{|S|}{2}\right)-P_i(b)$. More specifically,
either $\frac{|S|}{2}P_{t^*}\geq
\frac{1}{2}v_i\left(\frac{|S|}{2}\right)$ or
$u_i(b_i',b_{-i})+P_i(b)\geq
\frac{1}{2}v_i\left(\frac{|S|}{2}\right)$.  Additionally, observe that
when $\frac{|S|}{2}P_{t^*}\geq
\frac{1}{2}v_i\left(\frac{|S|}{2}\right)$, the utility of a player
from the deviation is at least $-P_i(b)$. Therefore, when
$\frac{|S|}{2}P_{t^*}\geq \frac{1}{2}v_i\left(\frac{|S|}{2}\right)$ it
is implied that $\frac{|S|}{2}P_{t^*}+u_i(b_i',b_{-i})+P_i(b)\geq
\frac{1}{2}v_i\left(\frac{|S|}{2}\right)$.  Hence, in any case we get:
\begin{equation}
  u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{|S|}{2}\right)-\frac{|S|}{2}P_{t^*}-P_i(b) \geq \frac{1}{2}v_i\left(\frac{|S|}{2}\right)-\frac{|S|}{2}p_{|S|/2}-P_i(b)
\end{equation}
Now we can use the simple fact that $\frac{|S|}{2}p_{|S|/2}\leq
\sum_{j=|S|/2}^{|S|}p_j\leq \sum_{j=1}^{|S|}p_j$. Thus we get:
$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{|S|}{2}\right)-\sum_{j=1}^{|S|}p_j-P_i(b)=\frac{1}{2}v_i\left(\frac{|S|}{2}\right)-\sum_{j\in S}p_j-P_i(b)$$
\end{proof}


\begin{thm}\label{thm:multi-unit} 
  The draft auction is a $(\frac{1}{4},2)$-smooth mechanism when items
  are identical and players have concave values over the units they
  acquired.
\end{thm}
\begin{proof}
  Consider a valuation profile $v$ and a bid profile $b$. Let $S_i^*$
  be the units allocated to player $i$ in the optimal allocation for
  profile $v$. By Lemma \ref{lem:multi-unit} we get that there exists
  a deviation mapping $b_i':B_i\rightarrow B_i$ for each player $i$
  such that for any strategy profile $b$, gives him utility at least:
\begin{equation}
  u_i(b_i'(b_i),b_{-i})\geq \frac{1}{2}v_i\left(\frac{|S_i^*|}{2}\right)-\sum_{j\in S_i^*}p_j - P_i(b)
\end{equation}
By the concavity of the valuation function we also have that
$v_i\left(\frac{|S_i^*|}{2}\right)\geq \frac{1}{2}v_i(|S_i^*|)$.
Last, summing over all players and observing that: $\sum_i \sum_{j\in
  S_i^*}p_j\leq \sum_{j}p_j=\sum_i P_i(b)$, we get the result.
\end{proof}

Thus we conclude that for the case of identical items, the price of anarchy of draft auctions with concave valuations
is at most $8$.

\subsection{Additive Bidders and Heterogeneous Items}

We next turn to simplest class of valuations over heterogeneous items, i.e. additive valuations. We show that the \emph{Core Deviating Lemma} implies a $\log(m)$ approximation. The key technical step is showing that any additive valuations can be
approximated to within a logarithmic factor by a \emph{constraint-homogeneous valuation}. Specifically, we show that for any additive valuation $v(\cdot)$ and for any set $S\subseteq [m]$, there exists a constraint-homogeneous valuation $\hat{v}$ such that $v(S)\leq O(\log(m))\cdot \hat{v}(S)$ and for any $T\subseteq [m]$: $\hat{v}(T)\leq v(T)$.

The idea is that we can group items in $S$, such that the valuation of a player for items within each group are within a factor of $2$ of each other, grouping together all items with value  less than a $1/m$ fraction of the highest valued item. Next we observe that there are $O(\log(m))$ such groups and thereby one of these groups must yield a total value to the bidder of at least a logarithmic fraction of his initial valuation for the whole set. Moreover, this group cannot be the last group of small items, since in total they are less valuable than the highest valued item. Thus we can consider the constraint homogeneous valuation whose target set is the most valuable among the above groups. Treating the items within each group as identical and with value equal to the minimum valued item in the group, can only result in a constant factor difference from the initial valuation. 

\begin{thm}\label{thm:additive}
  The draft auction is a $(\frac{1}{8\log(m)},2)$-smooth mechanism for
  additive bidders.
\end{thm}
\begin{proof}
  Consider a bidder $i$ with an additive valuation $v_i$. Let
  $\sjopt{i}$ be the set of items allocated to player $i$ in the
  optimal allocation. Sort the items in $\sjopt{i}$ according to the
  values $i$ has for them, $v_{i1} \geq v_{i2} \geq \ldots \geq
  v_{im_i}$. Consider the partition of items $\mathcal{P}$ where $I_1
  = \left\{j : v_{ij} \geq \frac{v_{i1}}{2}\right\}$, and more
  generally, for any $t\in \left[2, \log(m_i)\right]$

 \[I_t = \left\{j \mid \frac{v_{i1}}{2^{t-1}} > v_{ij} \geq
     \frac{v_{i1}}{2^t}\right\}\]


   Let the final set $I_f$ contain all the smallest items, $I_f =
   \left\{j : v_{ij} < \frac{v_{i1}}{m_i}\right\}$. Notice that the
   largest-valued item in $I_f$ has value at most $\frac{v_{i1}}{m_i}$
   and there are at most $m_i-1$ items in $I_f$, thus, $v_i(I_f) <
   v_{i1}$, and so $v_i(I_1) > v_i(I_f)$.  There are at most $\log(m)$
   sets in $\mathcal{P}$, so at least one of them has value at least
   $\frac{\svalopt{i}}{\log(v_{i1})}$.  If it is the case that $I_f$
   is such a set, then so is $I_1$.

Thus if we denote with $I_t^*=\arg\max_{t\in [1,\ldots,f-1]}v_i(I_t)$ we get that:
\begin{equation}
v_i(I_t^*) \geq \frac{v_i(\sjopt{i})}{\log(m_i)}
\end{equation}
Now consider the additive valuation $v_i'(\cdot)$ that assigns a value
of $\hat{v} =\min_{j\in I_t^*}v_{ij}$ to all items in $I_t^*$ and zero
to all other items. Valuation $v_i'(\cdot)$ and set $I_t^*$ satisfy
the premises of Lemma \ref{lem:multi-unit} and therefore there exist a
deviation mapping $b_i':B_i\rightarrow B_i$ such that, for any
strategy profile $b$:
\begin{equation}
u_i(b_i'(b_i),b_{-i};v_i')\geq \frac{1}{2}\frac{\hat{v}\cdot|I_i^*|}{2}-\sum_{j\in I_t^*}p_j-P_i(b)
\end{equation}
Now observe that a player's utility under $v_i(\cdot)$ is at least his
utility under $v_i'$. Additionally, since items in $I_t^*$ only differ
by a factor of $2$, we also know that $\hat{v}\cdot|I_i^*|\geq
\frac{v_i(I_i^*)}{2}$. Combining these two observation we get that
there exists a deviation mapping such that:
\begin{equation}
  u_i(b_i'(b_i),b_{-i};v_i)\geq \frac{1}{8}v_i(I_t^*)-\sum_{j\in I_t^*}p_j-P_i(b)\geq \frac{1}{8\log(m_i)}v_i(\sjopt{i})-\sum_{j\in \sjopt{i}}p_j-P_i(b)
\end{equation}
Adding the above inequalities gives the desired smoothness property.
\end{proof}

The latter smoothness theorem then implies that the price of anarchy of draft auctions is at most $16\log(m)$, for the
case of additive bidders.

\subsection{XOS Valuations}

Having proved the smoothness of the mechanism for general additive valuations, we now observe that a rephrasing of one
of the results in \cite{Syrgkanis2013}, is the following very useful Lemma about smooth mechanisms, which we prove here for completeness.

\begin{lem} If a mechanism in a combinatorial auction setting is $(\lambda,\mu)$-smooth for additive valuations then it is also 
$(\lambda,\mu)$-smooth for XOS valuations.
\end{lem}
\begin{proof}
  Consider an XOS valuation profile $v$. For each player $i$ let
  $S_i^*$ be his optimal allocation and let $v_i^*$ be the additive
  valuation that matches his value for his optimal allocation:
  i.e. $v_i(S_i^*)=v_i^*(S_i^*)$ and for any set $T$: $v_i(T)\geq
  v_i^*(T)$. Consider the additive valuation profile $v^*$ and for
  each player $i$, let $b_i':B_i\rightarrow B_i$ be the deviation
  mapping associated with the additive valuation, as designated by the
  smoothness for additive valuations.

  A players utility under $v_i$ is at least his utility under
  $v_i^*$. Additionally, the value of the optimal allocation under
  $v_i^*$ is at least $\opt(v)$, since the optimal allocation $S_i^*$
  is a feasible allocation that has value under $v^*$ of
  $\opt(v)$. Combining the two we get the smoothness property for $v$:
\begin{equation*}
  \sum_i u_i(b_i'(b_i),b_{-i};v_i)\geq \sum_i u_i(b_i'(b_i),b_{-i}; v_i^*)\geq \lambda \opt(v^*)-\mu \sum_i P_i(b)\geq \lambda \opt(v)-\mu \sum_i P_i(b)
\end{equation*}
\end{proof}

The latter Lemma essentially states that proving smoothness of a mechanism essentially boils down to proving it's smoothness 
only for the additive bidder setting. Combining the above Lemma with Theorem \ref{thm:additive} we directly get
smoothness of draft auctions for XOS valuations:
\begin{cor}\label{cor:xos} The draft auction is a
  $(\frac{1}{8\log(m)},2)$-smooth mechanism for XOS valuations.
\end{cor} 
This in turn implies that the price of anarchy of draft auctions for XOS valuations is at most $16\log(m)$.

\subsection{Subadditive Valuations}
\begin{lem}\label{thm:approx} 
  Suppose a mechanism in a combinatorial auction setting is
  $(\lambda,\mu)$-smooth when bidders have valuations drawn from some
  class $V$. Consider any class of valuations $V'$
  such that for any $v_i'\in V'$ there exists a $v_i\in V$ such that
  for any set of items:
\begin{equation}
   v_i(S)\leq v_i'(S)\leq  \beta \cdot v_i(S)
\end{equation}
then the mechanism is $(\frac{\lambda}{\beta},\mu)$-smooth
for the class $V'$.
\end{lem}
\begin{proof}
  Consider a valuation profile $v'=(v_1',\ldots,v_n')$ with $v_i'\in V'$. For each player
  $i$ let $v_i\in V$ be the corresponding valuation that
  $\beta$-approximates $v_i'$, as explained in the theorem statement. Let $b_i':B_i\rightarrow B_i$
  be the deviation associated with valuation profile
  $v=(v_1,\ldots,v_n)$ as designated by smoothness of the mechanism for valuation class $V$.  Then for any
  bid profile $b$:
\begin{align*}
  \sum_i u_i(b_i'(b_i),b_{-i};v_i') \geq~&  \sum_i u_i(b_i'(b_i),b_{-i};v_i) \geq  \lambda \opt(v)-\mu \sum_i P_i(b)\\
  \geq~& \frac{\lambda}{\beta}\opt(v')-\mu \sum_i P_i(b)
\end{align*}
\end{proof}

It is known that all subadditive valuations can be approximated by XOS
valuations in the sense of Theorem \ref{thm:approx} for $\beta=\log(m)$.  Thus by applying the above Lemma together with
corollary \ref{cor:xos} we get smoothness for subadditive valuations:

\begin{cor}\label{cor:subadditive}
  The draft auction is a $(\frac{1}{8\log^2(m)},2)$-smooth mechanism
  for subadditive valuations.
\end{cor}

This in turn implies that the price of anarchy of draft auctions for sub-additive valuations is at most $16\log^2(m)$.




%\begin{thm}\label{thm:multi-unit} 
%The draft auction is a $(\frac{1}{4},2)$-smooth mechanism when items are identical and players have concave values over the units they
%acquired.\end{thm}
%\begin{proof}
%Consider a valuation profile $v$ and a bid profile $b$. Let $k_i^*$ be the number of units allocated to player $i$ in the optimal allocation for profile
%$v$. Also let $p_j$ be the price that unit $j$ was sold under strategy profile $b$. Also re-order the index of the units such that $p_1\leq p_2\leq \ldots \leq p_m$. This is not necessarily the order at which they were sold. Let $t(j)$ be the auction at which item $j$ was sold and we denote with $P_t$ the price
%of auction $t$ under bid profile $b$.
%
%We also make the extra observation that the number of items that a player acquires at auction $t$, subject to winning, do not depend on the price of the auction since it is completely defined by the bid of the player. Additionally, a player doesn't learn anything else after the bidding phase. Thus we can think of each strategy as determining a bid $b_{it}$ and an amount of units $k_{it}$ for each auction $t$ that can depend on the history of play. 
%
%Consider the following deviation of player $b_i'$: let $b_i^*=\frac{1}{k_i^*}\cdot v_i\left(\frac{k_i^*}{2}\right)$ be half the average per unit value for $k_i^*/2$ items. At every auction $t$, as long as there are still $k_i^*/2$ items still remaining, he submits $b_{it}'=\max\left\{b_i^*, b_{it}\right\}$. If he wins with bid $b_i^*$ then he buys $k_i^*/2$ minus the number of units he has already acquired.  If he wins with a bid of $b_{it}$ he buys $k_{it}$. He does that until either he has won $k_i^*/2$ units or the auctions are over.
%
%The crucial observation is that as long as a player hasn't already acquired $k_i^*/2$ items then he is not affecting the game path created by strategy profile $b$ in any way, since either he behaved exactly as under $b$, by winning at his price under $b$ and getting the units  he would have got under $b$ or he won at a higher price, but then he acquired all the units needed to reach $k_i^*/2$ at the auction where he bid higher in the deviation. Thus the prices that he faces in all the auctions prior to having won $k_i^*/2$ items are the same as the prices under strategy profile $b$.
%
%First it is easy to observe that if player $i$ was obtaining at least $k_i^*/2$ items under $b_i$ then he is definitely winning $k_i^*/2$ items under $b_i'$. Moreover he is paying at most $\frac{k_i^*}{2} b_i^* + P_i(b)=\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)+P_i(b)$. Thus under this condition we get that
%the utility from the deviation is at least:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$$ 
%
%Thus we can assume that under $b_i$ player $i$ is winning less than $k_i^*/2$ units. Let $t^*$ be the first auction that was won at price $P_{t^*}\leq p_{k_i^*/2}$ under $b$ and not by bidder $i$. We know that such an auction must exist since there are $k_i^*/2$ units that are sold at a price
%less than $k_i^*/2$ and by the assumption on the limit of items won under $b_i$, some of them cannot be won by player $i$. Thus one such auction
%is the auction that this unit was sold at. 
%
%If player $i$ has already won $k_i^*/2$ units prior to $t^*$ then the same lower bound of $\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$ on the deviating utility holds. Thus we can assume that the player has not won $k_i^*/2$ items prior to $t^*$ and hence he is still bidding. Let $k_{i,<t^*}$ be the number of units acquired by player $i$ prior to $t^*$. Observe that by the definition of $t^*$ there are at least $k_i^*/2-k_{i,<t^*}$ units available
%for sale at that auction. This follows from the fact that for any auction $t<t^*$ for which $P_t\leq p_{k_i^*/2}$, we know that player $i$ was winning under $b_i$. Thus every unit that was sold prior to $t^*$ at a price of less than or equal to $p_{k_i^*/2}$ was sold to player $i$. There are $k_i^*/2$ units sold at a price $\leq p_{k_i^*/2}$ and the number of such units sold prior to $t^*$ is at most the number of total units allocated to bidder $i$ prior to $t^*$. Thus
%the number of available units available at $t^*$ is at least: $k_i^*/2-k_{i,<t^*}$.
%
%If $P_{t^*}<b_i^*$, then player $i$ is winning auction $t^*$. Since he was not winning $t^*$ under $b_i$, it must be that he is winning 
%$t^*$ with a bid of $b_i^*$. Thus at that auction he will buy every item needed to reach $k_i^*/2$ units. By the analysis in the previous paragraph,
%we know that there are still hat many units available for sale. Thus in this case he will win $k_i^*/2$ items and pay at most $\frac{k_i^*}{2} b_i^* + P_i(b)$. Therefore, we get that his utility from the deviation is also at least: $\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$.
%
%Thus the above analysis states that either $P_{t^*}\geq b_i^*$ or $u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$. More specifically,
%either $\frac{k_i^*}{2}P_{t^*}\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)$ or $u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$.
%Hence, in any case we get:
%\begin{equation}
%u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}P_{t^*}-P_i(b) \geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}p_{k_i^*/2}-P_i(b)
%\end{equation}
%Now we can use the simple fact that $\frac{k_i^*}{2}p_{k_i^*/2}\leq \sum_{j=k_i^*/2}^{k_i^*}p_j\leq \sum_{j=1}^{k_i^*}p_j$. Thus we get:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\sum_{j=1}^{k_i^*}p_j-P_i(b)$$
%
%By the concavity of the valuation function we also have that $v_i\left(\frac{k_i^*}{2}\right)\geq \frac{1}{2}v_i(k_i^*)$.
%
%Last, summing over all players and observing that: $\sum_i  \sum_{j=1}^{k_i^*}p_j\leq \sum_{j=1}^{m}p_j=\sum_i P_i(b)$, we get the result.
%\end{proof}






%\begin{thm} The draft auction is a $(\frac{1}{4},2)$-smooth mechanism for mutli-unit auctions with concave values.\end{thm}
%\begin{proof}
%Consider a valuation profile $v$ and a bid profile $b$. Let $k_i^*$ be the number of units allocated to player $i$ in the optimal allocation for profile
%$v$. Also let $p_j$ be the price that unit $j$ was sold under strategy profile $b$. Also re-order the index of the units such that $p_1\leq p_2\leq \ldots \leq p_m$. This is not necessarily the order at which they were sold. Let $t(j)$ be the auction at which item $j$ was sold and we denote with $P_t$ the price
%of auction $t$ under bid profile $b$.
%
%We also make the extra observation that the number of items that a player acquires at auction $t$, subject to winning, do not depend on the price of the auction since it is completely defined by the bid of the player. Additionally, a player doesn't learn anything else after the bidding phase. Thus we can think of each strategy as determining a bid $b_{it}$ and an amount of units $k_{it}$ for each auction $t$ that can depend on the history of play. 
%
%Consider the following deviation of player $b_i'$: let $b_i^*=\frac{1}{k_i^*}\cdot v_i\left(\frac{k_i^*}{2}\right)$ be half the average per unit value for $k_i^*/2$ items. At every auction $t$, as long as there are still $k_i^*/2$ items still remaining, he submits $b_{it}'=\max\left\{b_i^*, b_{it}\right\}$. If he wins with bid $b_i^*$ then he buys $k_i^*/2$ minus the number of units he has already acquired.  If he wins with a bid of $b_{it}$ he buys $k_{it}$. He does that until either he has won $k_i^*/2$ units or the auctions are over.
%
%The crucial observation is that as long as a player hasn't already acquired $k_i^*/2$ items then he is not affecting the game path created by strategy profile $b$ in any way, since either he behaved exactly as under $b$, by winning at his price under $b$ and getting the units  he would have got under $b$ or he won at a higher price, but then he acquired all the units needed to reach $k_i^*/2$ at the auction where he bid higher in the deviation. Thus the prices that he faces in all the auctions prior to having won $k_i^*/2$ items are the same as the prices under strategy profile $b$.
%
% Let $t^*$ be the first auction that was won at price $P_{t^*}\leq p_{k_i^*/2}$ under $b$. Observe that at that auction there are at least $k_i^*/2$ units available. 
%
%Consider the case where under $b$ player $i$ was not winning auction $t^*$. Thus if he wins auction $t^*$ under $b_i'$ it must be that he
%is winning it for a price of $b_i^*$. Suppose that $P_{t^*}\leq b_i^*$ then 
%if player $i$ hasn't already won $k_i^*/2$ items, he wins $t^*$ and gets the units remaining to reach $k_i^*/2$ units. Thus he gets utility at least  $$v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}b_i^*-P_i(b)\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b),$$ 
%since we also need to account for the auctions that player 
%$i$ won prior to $t^*$, at which he paid at most what he was paying under $b$ and the price that the player pays at $t^*$ is at most $\frac{k_i^*}{2}\cdot b_i^*=\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)$. If he had already won $k_i^*/2$ before $t^*$ then the same reasoning and bound will apply.
%
%Thus as long as player $i$ was not winning $t^*$ under $b_i$ we get that:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}P_{t^*}-P_i(b)\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}p_{k_i^*/2}-P_i(b)$$
%
%If player $i$ was winning $t^*$ under $b_i$, then he is still winning it under $b_i'$. If $b_{it}\leq b_i^*$, then 
%player $i$ will get $k_i^*/2$ units when winning, and therefore again we can bound the deviating utility by the latter bound. Same analysis
%will also apply even if $b_{it}\geq b_i^*$ but $k_{it^*}> k_i^*/2$.
%
%The only case that is left is when player $i$ was winning $t^*$ under $b_i$ but $b_{it}>b_i^*$ and $k_{it^*}<k_i^*/2$. In that case, consider
%the auction $t_2^*$ which is the first auction after $t^*$ that has a price of $P_{t_2^*}\leq p_{k_i^*/2}$. 
%Observe that since $k_{it^*}< k_i^*/2$ and by previous claims there are at least $k_i^*/2$ units available at auction $t^*$, all of 
%which where sold at a price lower than $p_{k_i^*/2}$ under $b$. Thus there exist $k_i^*-k_{it^*}$ unsold units after $t^*$ that are sold at a price of at 
%most $p_{k_i^*/2}$ and therefore there will exist an auction $t>t^*$ that is won at a price $P_t\leq p_{k_i^*/2}$ and such that $k_i^*-k_{it^*}$ 
%units are still available for sale. Thus $t_2^*$ is the first of these auctions and is well defined.
%
%If player $i$ was not winning auction $t_2^*$ under $b$ then if $P_{t_2}^*\leq b_i^*$ he gets utility at least:
%$$u_i(b_i',b_{-i})\geq v_i\left(\frac{k_i^*}{2}\right)-\left(\frac{k_i^*}{2}-k_{it^*}\right)b_i^*-P_i(b)\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)$$
%Thus as long as player $i$ is not winning $t_2^*$ under $b_i$, then the utility of the deviation is at least:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}P_{t_2^*}-P_i(b)\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}p_{k_i^*/2}-P_i(b)  $$
%If player $i$ is winning $t_2^*$ under $b_i$ and with a bid $b_{it_2^*}\leq b_i^*$ then the above bound also holds by similar analysis. Similarly, the bound
%holds if he was winning $t_2^*$ with $b_{it_2^*}>b_i^*$ and $k_{it_2^*}\geq k_i^*/2-k_{it^*}$.
%
%The only case that remains is when player $i$ was winning $t_2^*$ under $b_i$, and $b_{it_2^*}>b_i^*$ and $k_{it_2^*}< k_i^*/2-k_{it^*}$. 
%In that case we can similarly define $t_3^*$ as the first auction after $t_2^*$ that has price $P_{t_3^*}\leq p_{k_i^*/2}$. By similar reasoning as 
%to why $t_2^*$ was well defined, we can claim that $t_3^*$ is well defined. 
%
%We can do the same analysis for $t_3^*$ and all subsequent $t_r^*$, until the last condition in the above case analysis doesn't apply. Observe that 
%there will always exist a final $r$ such that the last condition wont apply, since if we do the above iteratively either we will reach an $r$ such that $k_i^*/2 -\sum_{r'<r}k_{it_r^*}\leq 1$ or we will have stopped at some previous $r$. But at that iteration we know that the player is always getting at least one item whenever winning under $b_i$ and therefore,
%the last case in the case analysis wont apply and we will stop. 
%
%The above analysis shows that the utility from the deviation is always lower bounded:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\frac{k_i^*}{2}p_{k_i^*/2}-P_i(b)$$
%Now we can use the simple fact that $\frac{k_i^*}{2}p_{k_i^*/2}\leq \sum_{j=k_i^*/2}^{k_i^*}p_j\leq \sum_{j=1}^{k_i^*}p_j$. Thus we get:
%$$u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-\sum_{j=1}^{k_i^*}p_j-P_i(b)$$
%
%By the concavity of the valuation function we also have that $v_i\left(\frac{k_i^*}{2}\right)\geq \frac{1}{2}v_i(k_i^*)$.
%Last, summing over all players and observing that: $\sum_i  \sum_{j=1}^{k_i^*}p_j\leq \sum_{j=1}^{m}p_j=\sum_i P_i(b)$, we get the result.
%
%%If player $i$ was winning some auction $t'\leq t$ under bid profile $b$ and let $t'$ be the 
%%smallest such $t'$. Then either he already won some auction $t''\leq t'$ or he is still winning $t'$ under bid profile $b_i'$ since he is bidding at least as high and his deviation up till timestep $t'$ is  transparent. Observe that if he is winning a $t''\leq t'$ under $b_i'$ but was not winning it under $b_i$ then
%%it is necessarily true that $\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)\geq b_{it''}$. Thus in that case player $i$ wins $\frac{k_i^*}{2}$ units and pays half his value for them
%%which means $u_i(b_i',b_{-i})\geq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)$. In the case where he didn't win some $t''\leq t'$ then he definitely wins $t'$ and therefore:
%%\begin{equation}
%%u_i(b_i',b_{-i})\geq v_i\left(\frac{k_i^*}{2}\right)-\max\left\{\frac{1}{2}v_i\left(\frac{k_i^*}{2}\right),b_{it}\right\}\geq  \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)-P_i(b)
%%\end{equation}
%%Thus, in any of the two cases, we get that if the player is winning some $t'\leq t$ under $b_i$ then the above lower bound on his utility must hold.
%%
%%Now we argue that a similar lower bound holds when player $i$ is not winning any auction $t'\leq t$ under $b_i$. Then when the auction $t$ arrives, the deviation of the player is transparent and therefore the player is facing a price of at most $p_{k_i^*/2}(b)$. If $p_{k_i^*/2}\leq \frac{1}{2}v_i\left(\frac{k_i^*}{2}\right)$ then the player will win and get utility:
%\end{proof}


==> unit-demand.tex <==
% !TEX root = draft.tex
Suppose each bidder is unit-demand: that is, each bidder $i$ has some
associated value with good $j$, denoted $v_{i,j}$, and for any set $S$
of goods, $v_i(S) = \max_{j\in S} v_{i,j}$. In this setting, the
single-item and many-item sequential draft auctions coincide: no
player will ever choose to pay for more than one item, given they've
won in the $t$th auction. Let $I_t$ denote the set of items remaining
for the $t$th auction.

\begin{fact}
\label{fact:fav}
  Suppose player $i$ wins at time $t$. Then, $i$ will select
  $\argmax_{j\in I_t} v_{i,j}$.
\end{fact}

Let $i_{I_t}$ denote $i$'s most preferred item from the set $I_t$.

\begin{fact}
\label{fact:one}
Consider a SPE that survives elimination of dominated strategies. If
player $i$ wins at round $t$ for price $p_t > 0$, $i$ has not won
prior to round $t$ and will not bid $b > 0$ after round $t$.
\end{fact}

\begin{proof}
  By Fact~\ref{fact:fav}, $i$ will select his favorite item in any
  round she wins. Thus, if $i$ won at time $t' < t$, $i$ will get no
  additional revenue from winning any future auction. So $i$ will not
  bid above $0$ at time $t$. 
\end{proof}


In light of Fact~\ref{fact:one}, the unit-demand case can be thought
of as the following game: in each round, a player wins the auction,
selects her most favorite item, and leaves the remaining auctions. Let
us rename the bidders so that bidder $i$ corresponds to the winner of
the $i$th auction. Similarly, let $p_i$ denote the winning price for
auction $i$ (which is won by bidder $i$).

\begin{obs}
  The prices $p_1, p_2, \ldots, p_m$ are weakly decreasing in a
  subgame perfect equilibrium, on the equilibrium path.
\end{obs}
\begin{proof}
  Suppose for sake of contradiction that there exists some $p_i <
  p_{i+1}$ at equilibrium. Then, bidder $i+1$ has strict incentive to
  win at time $i$: the set of available items at time $i$ is strictly
  larger, and the price is strictly smaller. This is a contradiction
  to the game being in a subgame perfect equilibrium.
\end{proof}

Despite all of this structure, draft auctions for unit demand bidders
may still be inefficient, even when all players agree on the relative
ordering of the items by their value. In the appendix, we show that
the price of anarchy is at least $209/177 > 1.22$ for unrestricted
unit-demand bidders. Here, we present an example of the inefficiency
which arises from the competition between agents.



The inefficiency of arbitrary subgame perfect equilibria suggests a
new conjecture: is the price of stability $1$? Here, we give an
example which shows the price of stability is strictly larger than
$1$, even when all bidders share the same ranking of the items by
value. Indeed, the example we give below also shows a setting \emph{in
  which no equilibrium is optimal}.

\begin{obs}
  The price of stability for unit-demand bidders in draft auctions is
  strictly larger than $1$, even when all bidders share the same
  ordering of items by value. This implies that the price of anarchy
  is also greater than $1$.
\end{obs}


\definecolor {processblue}{cmyk}{0.96,0,0,0}
\begin{figure}\label{fig:inefficent}
\begin{center}
\begin {tikzpicture}[-latex,scale=0.6,every node/.style={scale=0.6},auto ,node distance =2 cm and 4cm ,on grid ,
semithick , font=\small,
state/.style ={ circle ,top color =white , bottom color = processblue!20 ,
draw,processblue , text=blue , minimum width =.5 cm}]
\node[state] (C)
{$1$};
\node[state] (A) {$1$};
\node[state] (B) [below =of A] {$2$};
\node[state] (C) [below =of B] {$3$};
\node[state] (D)  [below =of C] {$4$};
\node[state] (E) [right = of A] {$a$};
\node[state] (F) [below =of E] {$b$};
\node[state] (G) [below =of F] {$c$};
\node[state] (H)  [below =of G] {$d$};
\path (A) edge [bend left =0, very near start] node[above] {$1$} (E);
\path (A) edge [bend left =0, very near start] node[above] {$1 - 2\epsilon$} (F);
\path (A) edge [bend left =0, very near start] node[below] {$1- 2\epsilon$} (G);

\path (B) edge [bend left =0, very near start] node[above] {$1$} (E);
\path (B) edge [bend left =0, very near start] node[above] {$1$} (F);

\path (C) edge [bend left =0, very near start] node[above] {$1$} (E);
\path (C) edge [bend left =0, very near start] node[above] {$1$} (F);
\path (C) edge [bend left =0, very near start] node[above] {$1- \epsilon$} (G);

\path (D) edge [bend left =0, very near start] node[above] {$1$} (E);
\path (D) edge [bend left =0, very near start] node[above] {$1$} (F);
\path (D) edge [bend left =0, very near start] node[above] {$2\epsilon$} (G);
\path (D) edge [bend left =0, very near start] node[above] {$2\epsilon$} (H);

\end{tikzpicture}
\end{center}
\caption{An example of inefficiency in draft auctions for unit-demand bidders}
\end{figure}

The example shown in Figure~\ref{fig:inefficent} has no equilibrium
where the optimal allocation is given. The optimal allocation is
$(1,a), (2,b), (3,c), (4,d)$, with a total weight of
$3+\epsilon$. Since the agents have the same ordering on items, item
$a$ will be selected first. So, for the optimal allocation to be an
equilibrium, $1$ must win the first round.  Then, assuming in the
subgame where $(1,a)$ is removed that the optimal allocation is
reached and solving for prices, the price vector for such an
allocation is $(1-2\epsilon, 1-2\epsilon, 0,0)$, where player $2$
price-sets in round $1$ and player $4$ price-sets in round
$2$\footnote{ We can ensure $2$ is the price-setter for player $1$ by
  slightly increasing the weight on the edges $(2,a)$. That way, $2$
  will have a slightly higher incentive to beat $1$ than $4$ has.}.
Thus, player $1$ gets utility $2\epsilon$ from winning the first
round.

Now, consider what happens if $1$ loses round $1$ to player $2$. If we
assume in any subgame, the optimal allocation is the one which is
made, the allocation in the subgame will be $(1,c), (3,b),
(4,d)$. Then, $3$ will pay $1-2\epsilon$, and $1$ will pay nothing,
for utility $1-2\epsilon$. So, if $1$ choses to lose to player $2$,
her utility is $1-4\epsilon$ higher than if she won round $1$.



%\begin{obs}
%  The pure-Nash PoA is 2 for unit-demand bidders.
%\end{obs}
%
%\begin{proof}
%  Consider an agent $i$ who gets the item $\jopt{i}$ in $OPT$. There are
%  2 cases: that $i$ wins in a round where $\jopt{i}$ has yet to be sold,
%  and where $i$ wins a round after $\jopt{i}$ has been sold. In case $1$,
%  $v_{i,j(i)} \geq \valopt{i}$ (since $i$ has the choice to take
%  $\jopt{i}$). In case 2, $v_{i,j(i)} \geq \valopt{i} -
%  p(\jopt{i})$. Summing up over all players, we have $SW_{EQ} \geq
%  SW_{OPT} - REV_{EQ}$. Thus, since $REV_{EQ} \geq SW_{EQ}$, by
%  individual rationality, $2SW_{EQ} \geq SW_{OPT}$.
%\end{proof}
%
%\begin{obs}  
%  The mixed-Nash PoA for unit-demand bidders is at most 2.
%\end{obs}
%\begin{proof}
%  Consider the deviation for player $i$ to bid $\valopt{i}/2$ at each
%  round until $\jopt{i}$ no longer is available. If $i$ wins, she gets
%  utility $\valopt{i}/2$, which implies $\exp[u_i] \geq \valopt{i}/2 \geq
%  \valopt{i}/2 - p_{\jopt{i}}$. If, on the other hand, she doesn't
%  win, this implies $p_{\jopt{i}} > \valopt{i}/2$, and so $\exp[u_i] \geq 0
%  > \valopt{i}/2 - p_{\jopt{i}}$. Thus, in either case
%
%  \[\exp_s[u_i(s)] \geq \frac{\valopt{i}}{2} - p_{\jopt{i}}\]
%
%  Summing up over all players, we have then that 
%\begin{eqnarray*}
% SW_{EQ} - REV_{EQ} & = & \sum_i \exp_s[u_i(s)] \\
%& \geq & \sum_i \frac{\valopt{i}}{2} - p_{\jopt{i}}\\
%& = & \frac{SW_{OPT}}{2} - REV_{EQ}
%\end{eqnarray*}
%
%Thus, $SW_{EQ} \geq \frac{1}{2} SW_{OPT}$.
%\end{proof}
%
%\begin{thm}The Bayes-Nash price of anarchy for unit demand bidders is $3$.
%\end{thm}
%\begin{proof}
%Consider a player $i$ with a value $v_i$. Let $j_i(b)$, be the item that player $i$ wins under a strategy profile $b$. We will show that for any item $j$, there exists a deviation $b_{ij}'$ such that, for any $b_{-i}$ and any strategy $b_i$ that is in the support of the equilibrium bid for player $i$ with value $v_i$:
%\begin{equation}
%u_i(b_{ij}',b_{-i})+\max_{k\neq i}b_{kj}(h_j(b)) +\frac{v_{ij_i(b)}}{2}\geq \frac{v_{ij}}{2}
%\end{equation}
%Where we denote with $h_j(b)$ the observed history of play at the auction where item $j$ was sold,  under strategy profile $b$.
%Consider the following deviation $b_{ij}'$ for player $i$: he switches to bidding $\frac{v_{ij}}{2}$ in all the auctions
%until $j$ is sold. If he wins he buys $j$ and drops out from then on.
%
%First consider the case where under $b$ player $i$ has not won any auction prior to $j$ being sold to some player under $b$. In this case by switching to 
%$b_{ij}'$ he is not affecting the history of play and therefore the prices that he faces at every auction up to $j_i^*$ are the same under $b$ and the same
%under $(b_{ij}',b_{-i})$, since he has not affected the (winner,price) announcement outcome. If $\max_{k\neq i}b_{kj}(h_j(b))<\frac{v_{ij}}{2}$ then the player definitely wins some auction before or at the time step that
%$j$ was sold. Thus he will get utility $u_i(b_{ij}',b_{-i})=\frac{v_{ij}}{2}$. Otherwise
%$\max_{k\neq i}b_{kj}(h_j(b))\geq \frac{v_{ij}}{2}$. Therefore in any case: $u_i(b_{ij}',b_{-i})+\max_{k\neq i}b_{kj}(h_j(b)) \geq \frac{v_{ij}}{2}$.
%
%In the case where player $i$ did win an auction under $b$, at or before the time step that $j$ was sold, then we know that he
%conditional on winning he is definitely picking the item with the highest value, since we assumed that $b_i$ is in the support of the equilibrium strategy for value $v_i$. Since
%$j$ is still available it must be that $v_{ij_i(b)}\geq v_{ij}$. Thus in this case we have: $\frac{v_{ij_i(b)}}{2}\geq \frac{v_{ij}}{2}$.
%
%Therefore in any case:
%\begin{equation}
%u_i(b_{ij}',b_{-i})+\max_{k\neq i}b_{kj}(h_j(b)) +\frac{v_{ij_i(b)}}{2}\geq \frac{v_{ij}}{2}
%\end{equation}
%
%Consider a Bayes-Nash equilibrium $s=(s_1,\ldots,s_n)$ where $s_i$ is a mapping from values $v_i$ to distributions over contingency plans $B_i$.
%Then for any value $v_i$ and for any item $j$ and any $b_i\in s_i(v_i)$:
%\begin{equation*}
%\E_{v_{-i}\sim F_{-i}, b_{-i}\sim s_{-i}(v_{-i})}\left[u_i(b_{ij}',b_{-i})\right] \geq\E_{v_{-i}\sim F_{-i}, b_{-i}\sim s_{-i}(v_{-i})}\left[\frac{v_{ij}}{2} -\max_{k\neq i}b_{kj}(h_j(b))-\frac{v_{ij_i(b)}}{2}\right]
%\end{equation*}
%Taking expectation over $b_i\sim s_i(v_i)$ the left hand-side is not affected and hence we get:
%\begin{equation*}
%\E_{v_{-i}\sim F_{-i}, b_{-i}\sim s_{-i}(v_{-i})}\left[u_i(b_{ij}',b_{-i})\right] \geq \E_{v_{-i}\sim F_{-i}, b\sim s(v)}\left[\frac{v_{ij}}{2} -\max_{k\neq i}b_{kj}(h_j(b))-\frac{v_{ij_i(b)}}{2}\right]
%\end{equation*}
%By equilibrium we have:
%\begin{align*}
%\E_{v_{-i}\sim F_{-i}, b\sim s(v)}\left[u_i(b)\right]\geq~& \E_{v_{-i}\sim F_{-i}, b_{-i}\sim s_{-i}(v_{-i})}\left[u_i(b_{ij}',b_{-i})\right]\\
%\geq~& \E_{v_{-i}\sim F_{-i}, b\sim s(v)}\left[\frac{v_{ij}}{2} -\max_{k\neq i}b_{kj}(h_j(b))-\frac{v_{ij_i(b)}}{2}\right]
%\end{align*}
%Taking expectation over $v_i$ we get:
%\begin{equation*}
%\E_{v,b\sim s(v)}\left[u_i(b)\right]\geq \E_{v, b\sim s(v)}\left[\frac{v_{ij}}{2} -\max_{k\neq i}b_{kj}(h_j(b))-\frac{v_{ij_i(b)}}{2}\right]
%\end{equation*}
%
%For any valuation profile $v$ let $j_i^*(v)$ be the optimal item for player $i$ under valuation profile $v$. Now consider a hypothetical valuation profile $w$. Then the above inequality holds for $j_i^*(v_i,w_{-i})$ for each player $i$. Applying
%it for the above item taking expectation over $w\sim F$ and summing over all players we get: 
%\begin{align*}
%\E_{v,b\sim s(v)}\left[\sum_i u_i(b)\right]\geq~& \sum_i\E_{v,w, b\sim s(v)}\left[\frac{v_{ij_i^*(v_i,w_{-i})}}{2}\right] -\sum_i\E_{v,w,b\sim s(v)}\left[\max_{k\neq i}b_{kj}(h_j(b))\right]-\sum_i \E_{v,b\sim s(v)}\left[\frac{v_{ij_i(b)}}{2}\right]\\
%\geq~& \sum_i\E_{v_i,w_{-i}}\left[\frac{v_{ij_i^*(v_i,w_{-i})}}{2}\right]-\sum_i\E\left[\max_{k}b_{kj}(h_j(b))\right]-\frac{1}{2}\E_{v,b\sim s(v)}\left[SW(b)\right]\\
%=~& \sum_i\E_{w}\left[\frac{v_{ij_i^*(w)}}{2}\right]-\sum_i\E\left[p_j(b)\right]-\frac{1}{2}\E_{v,b\sim s(v)}\left[SW(b)\right]\\
%\end{align*}
%\end{proof}





 

==> xos.tex <==

Consider the class of valuation functions $XOS$, where each function
$f\in XOS$ can be represented as the maximum of some $k$ additive
functions:

\[f(S) = \max\left(\sum_{j\in S}v_{1j}, \ldots, \sum_{j\in S}v_{kj}\right)\]

Our result for additive bidders can extend to this class as well.

\begin{thm}\label{thm:xos}
  Suppose the set of bidders are $XOS$. Then, the pure PoA is
  $O(\log(m))$.
\end{thm}

\begin{proof}
  Consider a fixed bidder $i$. Let the bundle $i$ received at $OPT$ be
  denoted as $\sjopt{i}$. If we consider $v_i$ in its representation as above

  \[v_i(S) = \max\left(\sum_{j\in S} w_{1j}, \ldots, \sum_{j\in S}
    w_{kj}\right)\]

  then $v_i(\sjopt{i}) = \sum_{j\in \sjopt{i}} w_{tj}$ for some $t\in
  [1,k]$. That is, $i$'s value for the set $\sjopt{i}$ \emph{is at
    least additive on all of its subsets}. This implies that any lower
  bound on the utility of a given deviation for additive bidders also
  holds for $XOS$ bidders.

  Thus, since by Lemma~\ref{lem:adddev} there is a deviation which
  achieves at least $\frac{\svalopt{i}}{4\log(m)} - \sum_{j\in J(i)}
  p_j - \sum_{j\in \jopt{i}} p_j$, there is a deviation for any XOS
  bidder which achieves at least this much utility.
\end{proof}

